Fairness-Aware Online Personalization

Decision making in crucial applications such as lending, hiring, and college admissions has witnessed increasing use of algorithmic models and techniques as a result of a confluence of factors such as ubiquitous connectivity, ability to collect, aggregate, and process large amounts of fine-grained data using cloud computing, and ease of access to applying sophisticated machine learning models. Quite often, such applications are powered by search and recommendation systems, which in turn make use of personalized ranking algorithms. At the same time, there is increasing awareness about the ethical and legal challenges posed by the use of such data-driven systems. Researchers and practitioners from different disciplines have recently highlighted the potential for such systems to discriminate against certain population groups, due to biases in the datasets utilized for learning their underlying recommendation models. We present a study of fairness in online personalization settings involving the ranking of individuals. Starting from a fair warm-start machine-learned model, we first demonstrate that online personalization can cause the model to learn to act in an unfair manner if the user is biased in his/her responses. For this purpose, we construct a stylized model for generating training data with potentially biased features as well as potentially biased labels and quantify the extent of bias that is learned by the model when the user responds in a biased manner as in many real-world scenarios. We then formulate the problem of learning personalized models under fairness constraints and present a regularization based approach for mitigating biases in machine learning. We demonstrate the efficacy of our approach through extensive simulations with different parameter settings. Code: https://github.com/groshanlal/Fairness-Aware-Online-Personalization

==> mitigation_strategies.tex <==
\subsection{Bias Mitigation Strategies} \label{sec:mitigation}
We next present a brief overview of some of the mitigation strategies for bias in machine learning. We start with independence based fairness condition.

\TODO{Shorten / Better present the related work below}
A method for certifying and removing disparate impact in data is proposed in ~\cite{feldman_2015}. This is achieved by transforming the data such that the cumulative distribution conditioned on the protected attribute maps to some distribution independent of the protected attribute.

In~\cite{kamiran_2010}, the authors
present interesting approaches which makes the training data look as if it satisfies independence constraints. One approach suggested by them is to up-sample/down-sample each training data point such that the training data labels appear to be independent of the protected attribute. Another approach suggested by them is to promote/demote results of certain training data points which are at the boundary of the decision curve such that the output of the model appears to be independent of the protected attribute during training time.

In~\cite{zemel_2013}, the authors introduced a learning based approach which transforms data points to a fair space while trying to maintain as much information as possible about the data points (be able to re-construct the data points from the transformed space sufficiently well) and enforcing statistical parity in the transformed space. Using such a transformed space for machine learning applications results in more fair outcomes.

In recent years, the deep learning community has employed generative methods to generate fair representations of data. Two of the popular generative methods in deep learning are Generative Adversarial Networks (GANs) introduced by Goodfellow and Variational Autoencoders introduced by Kingma et al. GAN based approach to generate fair representations was introduced by Edwards et al. The GAN is trained such that the protected attribute cannot be derived from the fair transformation. VAE based approach to generate fair representations was introduced by Louizos et al. \TODO{Cite these papers, and rewrite} 

We now discuss some popular mitigation methods for conditional independence based fairness condition. To ensure equal true positive rates and false positive rates, in~\cite{hardt_2016}, the authors propose drawing separate ROC curves for each protected group and choosing the hyper-parameters corresponding to the point where they intersect.

The special case of jointly Gaussian variables is investigated in~\cite{woodworth_2017}. The authors show that conditional independence based fairness conditions on jointly gaussian variable leads to linear predictors. Further, optimizing linear predictors with fairness conditions leads to a convex optimization problem.


